Gemini: A Grammar and Recommender System for AnimatedTransitions in Statistical Graphics

Animated transitions help viewers follow changes between related visualizations. Specifying effective animations demands significant effort: authors must select the elements and properties to animate, provide transition parameters, and coordinate the timing of stages. To facilitate this process, we present Gemini, a declarative grammar and recommendation system for animated transitions between single-view statistical graphics. Gemini specifications define transition "steps" in terms of high-level visual components (marks, axes, legends) and composition rules to synchronize and concatenate steps. With this grammar, Gemini can recommend animation designs to augment and accelerate designers' work. Gemini enumerates staged animation designs for given start and end states, and ranks those designs using a cost function informed by prior perceptual studies. To evaluate Gemini, we conduct both a formative study on Mechanical Turk to assess and tune our ranking function, and a summative study in which 8 experienced visualization developers implement animations in D3 that we then compare to Gemini's suggestions. We find that most designs (9/11) are exactly replicable in Gemini, with many (8/11) achievable via edits to suggestions, and that Gemini suggestions avoid multiple participant errors.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> future.old.tex <==


\section{Conclusion \& Future Work}

In this paper, we presented Gemini, a declarative grammar for authoring animated transition between single-view statistical graphics specified in the Vega grammar. We began by setting design goals for an animated transition grammar. We reviewed alternate strategies and presented the primitives of the grammar with backing rationales. Three examples evaluate the expressiveness of the grammar, and the usage scenario shows how Gemini can facilitate the animation design process.
% We now discuss the automation of animated transitions enabled by Gemini and the implementation of Gemini compiler. 

A great deal of future work remains. First, the expressiveness of Gemini needs to be further extended. To express the transitions of more varied charts, for example, multi-view charts and geographic charts, the grammar needs to extend the steps to support new components and changes like headers and mark groups, or geographic projections. In addition, supporting temporary scales seems promising. For example, when points move from a range of $[0,1]$ to $[11,12]$, it might be better to set a temporary scale as $[0,12]$ before moving the points, such that readers can see the 10-plus-length movements of the points. Similarly, allowing intermediate data states seems helpful as it can stage the transition with complicated data transforms (\eg aggregation while filtering). 

In terms of usability, supporting interactions with the generated animated transitions is promising. Currently Gemini assumes that users will only play a transition from the start and reset at the end. However, animated transitions may also interact with various user inputs; for example, the position of the mouse scroll controlling the progress of the animated transition~\cite{R2D3}.

In addition, Gemini can provide a high-level representation for computers to perform search and recommendation over a space of animation designs. For example, diverse compositions of the sync and concat operations can produce multiple timelines of given steps.
However, Gemini provides a combinatorial search space for possible designs per animated transition, which costs too much to comprehensively evaluate. Similar to the Draco knowledge base for visualization design~\cite{draco}, a knowledge base incorporating constraints and best practices for animation design could enable efficient synthesis of animated transition designs. Open challenges include how to formalize animation guidelines~\cite{anim_transition, tversky} within constraint programming systems. Gemini's autoScaleOrder feature is a first step in this direction.

% For example, if a system split the given transition into five distinct steps, they can be composed into 541 possible timelines by only varying the sync and concat operations. On top of these choices, the systems should consider how to set the timing of each step. In response to this, Gemini demands the rules excluding incongruent animation designs as the autoScaleOrder excludes the designs occurring data overflow. 

% In terms of choosing the best design among the candidate designs, Gemini can enable systematic evaluation if the animation design guidelines can incorporate with Gemini grammar.  For example, if the design guideline about the staging technique suggests the maximum number of components that can change simultaneously, Gemini compiler can parse the animated transition specification and check if the design validates the guideline or not.

In conclusion, we see Gemini as both a practically useful grammar in its own right and as a promising vehicle for higher-level tools that can help synthesize and evaluate animated transition designs. The Gemini compiler and examples will be made available as open source software at \emph{anonymized URL}.

% more research is needed to fulfill this Gemini's possibility. Including Congruence and Apprehension principals\cite{tversky, anim_transition}, when the studies are interpreted in the frame of Gemini grammar, Gemini can search for the feasible space and tune the evaluation to recommend the best design. 

% n=1 -> 1
% n=2 -> 3
% n=3 -> 13
% n=4 -> 75 A_(k,n) = k * (A_(k,n-1) + A_(k-1, n-1)) when k>n A_(k,n)=0, A_(n,n) = n!, A_(1,n) = 1;

\section{Acknowledgements}

Anonymized for the submission.



% \section{Conclusion}


==> implementation.tex <==
\section{Implementation of Gemini Compiler}

The Gemini compiler requires both a visualization library and an animation library for the chosen rendering platform (\eg SVG, HTML Canvas). The visualization library renders visualizations on the platform and enables Gemini to parse the visualizations into data, scales, and visual encoding per graphic component (\eg mark, axis, legend). With the parsed results, Gemini can compute component-wise differences between the start and end of each step. The animation library supports interpolation between graphic elements on the platform, using the extracted differences.

Our current prototype compiler is implemented for SVG elements, using Vega and D3 as the visualization and animation libraries, respectively. It is limited to support for axis, view, pause, and mark components, over Vega's line, rectangle, and symbol mark types. 
%the remain parts are extendable by adding more engineering resources along with our implementation.
The compiler is composed of three key components: \code{Scheduler}, \code{Change Fetcher}, and \code{Actuator}. First, the \code{Scheduler} parses the timeline block into the composing steps with start and end times. The \code{Scheduler} recursively applies a function on every block with the context of its parent block to calculate the times. If any concat block has an enumerator, it enumerates the concat with the corresponding filtering values and the divided timings. If any concat block has autoScaleOrder, it permutes the concat's children blocks and stores the possible orders. 

After the \code{Scheduler} returns the schedule of steps, the \code{Change Fetcher} calculates and fetches the initial and final component states (such as data, encoding, scales, signals, and mark-type) of each step. This calculation involves 1) the start and end visualizations, 2) user-provided step changes, and 3) the previous state of the component. The initial component state of each step continues from the final state of the previous step of the component or gets initialized from the start visualization. The final state of the step is derived from the end visualization by default. If there are user-provided step changes suppressing parts of the changes, these parts of the state retain their initial values. If users specify an encoding change, this overwrites the initial encoding state. For data changes, we retrieve start and end data sets of the component using the Vega API and calculate changes as described in Step Change section. During the calculation, we also check if the data overflows their scale domains and alternate the schedule to a valid order when autoScaleOrder is set.

The schedule with fetched changes is wrapped with an \code{Actuator} and returned to users as a playable object. When users play the object, the \code{Actuator} executes the steps with the fetched states according to the schedule. It uses D3 to select the rendered SVG elements and interpolate between step start and end states. As different component types (\eg, mark, axis, view) and mark types (\eg, rectangle, symbol, line) have different SVG element hierarchies, we apply different actuation functions for each type.

For improved performance, the Gemini compiler should be updated to deal with computational complexity stemming from the size of the data and steps. The steps involving data changes induce data joins between two data sets. The complexity increases with use of enumerators and the autoScaleOrder feature. The enumerators iterate data join processes for each enumerated step, and the autoScaleOrder makes Gemini search until it finds a valid order of the given concat block among all possible permutations. For example, the Gemini prototype compiler takes about 5 seconds for compiling \designC{} in \autoref{fig:usage_scenario} by a laptop computer when it enumerates 4 more stages, which can be instantly playable in D3 implementation. Future optimizations to the Gemini compiler\,---\,such as indexing for data joins and dynamic programming to validate the permutations for the autoScaleOrder\,---\,could provide better performance.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

